On the detection of internal interfacial layers in turbulent flows

A novel approach to identify internal interfacial layers, or IILs, in wall-bounded turbulent flows is proposed. Using a Fuzzy Cluster Method (FCM) on the streamwise velocity component, a unique and unambiguous grouping of the Uniform Momentum Zones is achieved, thus allowing the identification of the IILs. The approach overcomes some of the key limitations of the histogram-based IIL identification methods. The method is insensitive to the streamwise domain length, can be used on inhomogeneous grids, uses all the available flow field data, is trivially extended to three dimensions, and does not need user-defined parameters (e.g. number of bins) other than the number of zones\add{. The number of zones can be automatically determined by an \emph{a priori} algorithm based on a Kernel Density Estimation algorithm, or KDE.} The clustering approach is applied to the turbulent boundary layer (experimental, planar PIV) and channel flow (numerical, DNS) \add{at varying Reynolds numbers}. \modify{The interfacial layers are characterized by a strong concentration of spanwise vorticity, with the outer-most layer located at the upper edge of the log-layer. The three-dimensional interface identification reveals a streak-like organization; we show that the organization of the IILs is correlated to the underlying wall-bounded turbulent structures. }

==> JFM2018_experiment.tex <==
\section{Experimental and numerical databases}\label{sec:experiment}
Two snapshots of incompressible channel flow DNS data simulated by
\citet{del2004scaling} were examined in present study. The evolution
of wall-normal vorticity \(\omega_y\) and the laplacian of wall-normal
velocity \(\nabla^2 V\) are integrated in the Fourier space using
Fourier expansion in the periodic stream-wise and span-wise direction
and Chebychev polynomials in the wall-normal direction. The Reynolds
number based on the friction velocity \(u_{\tau}\)
\(Re_{\tau}=\frac{u_{\tau}h}{\nu}\) is 950 and 550 ,respectively,
where \(\nu\) denotes the kinematic viscosity. The first utilized
channel flow data(\(Re_{\tau}=950\)) is comparable to the PIV
measurement by \citet{kwon2014quiescent} where \(Re_{\tau}\approx
1000\). The size of both simulations is \(Lx=8\pi\) in stream-wise,
\(Ly=2\) in wall-normal direction and \(Lz=3\pi\) in span-wise
direction which are non-dimensionalized by the channel half-height
\(h\). The large simulation box enables the examination of the very
large energetic structure which scale is proportional to \(h\) that
cannot be captured by other simulations with a smaller
domain. Previous study of interfacial layers between
UMZs\citep{de2017interfaces} using the flow field measured by PIV
usually covers a field view of around \(2-3\delta\), so the variations
of the interfacial layers cannot be examined carefully. However, the
large simulation here make the investigation of the stream-wise and
span-wise variation possible. Other flow parameters are summarized in
\ref{tab:piv} and further details can be found in
\citet{del2004scaling}. Besides the channel flow data, the velocity
field measured by PIV \citep{tomkins1998structure} was also utilized
to validate and compare \citet{adrian2000vortex}'s histogram method
and current cluster method. The measurement details are also
summarized in \ref{tab:piv}.

\begin{table}
 \begin{center}
\def~{\hphantom{0}}
 \begin{tabular}{cccccccc}
  & \(\Rey_{\tau}\) & \(L_x\) &\(L_y\) &\(L_z\) &\(\Delta x^+\) &\(\Delta y^+\)&\(\Delta z^+\) \\
  TBL PIV &  &  & & & & & \\
  Channel DNS & & & & & & &
 \end{tabular}
 \caption{Flow parameters of \citet{tomkins1998structure}'s PIV measurements}
 \label{tab:piv}
\end{center}
\end{table}
